DS-Sync: Addressing Network Bottlenecks with Divide-and-Shuffle Synchronization for Distributed DNN Training

Bulk synchronous parallel (BSP) is the de-facto paradigm for distributed DNN training in today's production clusters. However, due to the global synchronization nature, its performance can be significantly influenced by network bottlenecks caused by either static topology heterogeneity or dynamic bandwidth contentions. Existing solutions, either system-level optimizations strengthening BSP (e.g., Ring or Hierarchical All-reduce) or algorithmic optimizations replacing BSP (e.g., ASP or SSP, which relax the global barriers), do not completely solve the problem, as they may still suffer from communication inefficiency or risk convergence inaccuracy. In this paper, we present a novel divide-and-shuffle synchronization (DS-Sync) to realize communication efficiency without sacrificing convergence accuracy for distributed DNN training. At its heart, by taking into account the network bottlenecks, DS-Sync improves communication efficiency by dividing workers into non-overlap groups to synchronize independently in a bottleneck-free manner. Meanwhile, it maintains convergence accuracy by iteratively shuffling workers among different groups to ensure a global consensus. We theoretically prove that DS-Sync converges properly in non-convex and smooth conditions like DNN. We further implement DS-Sync and integrate it with PyTorch, and our testbed experiments show that DS-Sync can achieve up to $94\%$ improvements on the end-to-end training time with existing solutions while maintaining the same accuracy.

==> sections/acknowledge.tex <==
\section*{Acknowledgment}
 This work is supported in part by the Hong Kong RGC TRS T41-603/20-R, GRF-16215119, GRF-16213621 and a Huawei research grant. We thank Li Chen and Hong Zhang for the helpful discussion and the anonymous
reviewers for their constructive feedback and suggestions. Kai Chen is the corresponding author of the paper.

==> sections/introduction.bak2.tex <==
\section{Introduction}


With growing training data volume and model complexities, deep learning (DL) has dominated in many fields like computer vision(CV)~\cite{DBLP:conf/cvpr/HeZRS16,DBLP:conf/bmvc/ZagoruykoK16} and natural language processing(NLP)~\cite{DBLP:conf/naacl/DevlinCLT19}. To save training time and budget, it is a common practice for DL to conduct distributed machine learning(DML) on the large-scale shared GPU cluster~\cite{DBLP:conf/usenix/JeonVPQXY19,DBLP:conf/osdi/ZhaoHYZYZYLWXW20} or cloud~\cite{DBLP:conf/mlsys/LuoWKCN20,DBLP:conf/osdi/XiaoBRSKHPPZZYZ18}. DML usually distributes data batches to multiple workers of the cluster or cloud to parallelize the computation. Then synchronization accumulates and averages local gradients of all workers to update the model iteration by iteration. The synchronization overhead consists of communication costs and waiting time for the slowest worker, aka straggler. There is less computation cost with more workers but more intensive communication and a higher probability of stragglers.

Synchronization often suffers from network bottlenecks on a shared cluster or cloud due to network heterogeneity and contention. With many tasks running simultaneously, GPU resource allocation is in the fragmentation~\cite{DBLP:conf/usenix/JeonVPQXY19,DBLP:conf/osdi/ZhaoHYZYZYLWXW20,DBLP:conf/mlsys/LuoWKCN20} so that workers are often in different racks and even pods~\cite{DBLP:conf/mlsys/ChoF0H19, DBLP:conf/osdi/ZhaoHYZYZYLWXW20,DBLP:conf/mlsys/LuoWKCN20}. Some links have to cross upper-level switches, while most links are within the same region. Different DML tasks may also co-locate on the same physical node and compete for the network interface card(NIC)~\cite{DBLP:conf/osdi/ZhaoHYZYZYLWXW20,DBLP:conf/mlsys/WangVPTDS20}. Therefore, DML tasks running simultaneously can hardly avoid sharing upper-level links and NICs, which results in some workers delayed by network bottlenecks. E.g., In the EC2 cloud, slow pairs of workers can have only the half network throughput of the fast pairs~\cite{DBLP:conf/mlsys/LuoWKCN20}. 
%Since the fragmentation and multiple DML tasks exist for a long time, persistent stragglers due to network bottlenecks last for many iterations instead of only one. 

Prior works about synchronization do not handle network bottlenecks very well. There are two categories of related works, namely system-level optimization and algorithmic optimization. Many system works~\cite{DBLP:conf/cluster/MamidalaLP04,DBLP:conf/ipps/PatarasukY07,DBLP:conf/osdi/JiangZLYCG20, DBLP:conf/ppopp/AwanHHP17,DBLP:conf/usenix/ZhangZXDHLHWXX17,DBLP:conf/infocom/BaoPCW20,DBLP:conf/sosp/PengZCBYLWG19} make too ideal assumption of uniform network links. Hierarchical Allreduce~\cite{DBLP:conf/mlsys/ChoF0H19, DBLP:conf/mlsys/LuoWKCN20} uses sequential communications instead, but it is sub-optimal due to the in-cast problem~\cite{DBLP:conf/mlsys/LuoWKCN20} or not full use of bandwidth~\cite{DBLP:conf/mlsys/ChoF0H19}. The algorithmic optimizations including Asynchronous parallel (ASP)~\cite{asp}, stale synchronous parallel(SSP)~\cite{nips:ssp,DBLP:conf/ppopp/LiBGAH20}, and gossip algorithms~\cite{DBLP:conf/nips/LianZZHZL17,DBLP:conf/icml/AssranLBR19} relax synchronization conditions. Nevertheless, they only focus on stragglers due to stochastic events like system interruption, expecting that stragglers will catch up very soon. However, workers delayed by network bottlenecks accumulate staleness to a high level. The high-level staleness brings two problems: (1) slower convergence speed and even failures~\cite{DBLP:conf/iclr/DaiZDZX19} (2) frequently global waiting in SSP and gossip algorithms. %Additionally, gossip algorithms also have the in-cast problem in the overlapped neighborhoods. 
All previous works only attempt to localize bottlenecks or stragglers, but they ignore the possibility of speeding up the workers delayed by network bottlenecks.

 To this end, we propose Divide-and-Shuffle Synchronization (DS-Sync) to alleviate network bottlenecks by reducing its group size to synchronize. DS-Sync is motivated by the observation that synchronizing more workers takes more time(details in Section~\ref{sec:sync_scale}). It divides all workers into independent groups of different sizes to synchronize in parallel. It decouples network bottlenecks from other groups and keeps related workers in the smaller group, while other normal workers form larger groups to avoid idle waiting. With less latency and transfer cost, small groups with network bottlenecks can catch up and may keep the same pace with other large groups consisting of normal workers. 

Shuffling is the critical ingredient for DS-Sync to maintain convergence, which we formally prove in non-convex and smooth situations like DNNs in Sec~\ref{sec:convergence}. In every iteration, DS-Sync shuffles the group members in a designed pattern. Therefore, any worker can synchronize parameters with unseen workers from other groups in the last iteration. Intuitively, shuffling enables every worker to get the global update information from all workers in certain iterations instead of every iteration. We can further extend the stochastic weight average(SWA)~\cite{DBLP:conf/uai/IzmailovPGVW18} to ensemble the diverse local models for better generalization performance. In Fig~\ref{fig:ds_sync}, we compare our DS-Sync with bulk synchronization(BSP) and gossip and illustrate its advantages of speeding up workers affected by network bottlenecks to improve system throughput.

 \begin{figure*}[ht]
  	\centering

  	\includegraphics[scale=0.55]{figures/ds_sync.pdf}
  	\caption{comparison in two racks(Worker 0-3 in one rack and 4-7 in the other)  with upper-level link(red dash line) and in-cast workers(red number): (a) Hierarchical AllReduce~\cite{DBLP:conf/mlsys/ChoF0H19,DBLP:journals/corr/abs-1807-11205} have three stages pipeline of intra- or inter- rack communication: reduce, Allreduce and broadcast. The workers 0 and 4 in all three stages suffer from the in-cast problem. (b) Gossip Algorithm breaks the global synchronization into multiple chained local ones. However, the upper-level link is competed by two connections. The accumulated staleness finally affects all chained workers. Moreover, the overlapped neighbourhood also suffers from the in-cast problem. (c) DS-Sync divides workers into independent groups without overlapping and shuffles group members every iteration. It reduces transfer delay and latency for the influenced workers by forming a smaller group to catch up with normal workers. }
  \label{fig:ds_sync}
  \end{figure*}
  
 We have implemented DS-Sync in the Pytorch framework and conducted comprehensive experiments. To verify its improvements, we conduct experiments on the popular models and datasets in CV and NLP. Empirical measurement shows DS-Sync can achieve speed up as high as two times over baselines. 

Overall, we propose DS-Sync to reduce DML training wall-time by alleviating network bottlenecks and speeding up delayed workers. In summary,  DS-Sync makes 3-fold contributions as follows:
\begin{enumerate}
	\item We propose the DS-Sync that divides and shuffles workers into parallel groups to synchronize independently instead of the global synchronization. It schedules workers to form groups of different sizes and keeps network bottlenecks and related workers in the smaller groups to catch up. 
    \item We formally prove that DS-Sync converges properly on training data in non-convex and smooth situations like DNN. If not much better, the extended ensemble strategy at least helps maintain the same generalization performance on test data.
    \item We implement DS-Sync in the PyTorch framework and verify the improvements by comprehensive experiments. Empirical study shows DS-Sync can achieve speed up as high as two times compared with baselines.
 \end{enumerate}

==> sections/introduction.tex.bak.tex <==
\section{Introduction}
The success of machine learning relies on the available large datasets and complex deep neural network(DNN). Due to the growing data volumes and model complexities, training DNN can take days and even weeks. Therefore, Distributed Machine Learning(DML) usually distributes data batches over different workers of a GPU cluster or cloud to parallelize the computation. Then global synchronization accumulates and averages all workers' local gradients to update the global model iteration by iteration. However, synchronizing massive workers means not only intensive communication but also long waiting time for stragglers. The synchronization can usually be the system bottleneck, especially on a crowded GPU cluster or cloud shared by many DML tasks. 

There are two categories of previous related works. One approach is system-level optimization. Some works~\cite{DBLP:conf/cluster/MamidalaLP04,DBLP:conf/ipps/PatarasukY07,DBLP:conf/osdi/JiangZLYCG20} explore proper communication topologies for optimal bandwidth utilization. Recent works~\cite{DBLP:conf/ppopp/AwanHHP17,DBLP:conf/usenix/ZhangZXDHLHWXX17,DBLP:conf/infocom/BaoPCW20,shiexploiting, DBLP:conf/sosp/PengZCBYLWG19} consider overlapping computation and communication with sophisticated pipeline and schedule. However, these works make ideal assumptions about the network, which cannot hold in the real network environment of the crowded platforms. Some works~\cite{DBLP:conf/mlsys/ChoF0H19, DBLP:conf/mlsys/LuoWKCN20} also propose hierarchical AllReduce for heterogenous networks, but it is sub-optimal because of the serial synchronizations and low network utilization. 

The other line of works on algorithmic optimization attempt to relax the synchronization constrains. Some early works~\cite{asp} use fully asynchronous parallel (ASP) computations to get rid of idle waiting directly.  Stale synchronous parallel(SSP)~\cite{nips:ssp,DBLP:conf/ppopp/LiBGAH20} allows fast workers to move on with some stale bounds. Gossip based algorithms~\cite{DBLP:conf/nips/LianZZHZL17,DBLP:conf/icml/AssranLBR19} break the global AllReduce into chained local communications in the neighbourhoods to relay updates iteratively. Those works may absorb stochastic stragglers by hoping they can catch up later. However, recent studies~\cite{arxiv:toward} show that stale gradient slow down convergence and even fail it sometimes, especially when training non-convex DNNs with advanced optimizers considering momentum. Additionally, the gossip based algorithm suffers from in-cast problem due to overlapped neighbourhoods. Most importantly, these works cannot handle persistent stragglers resulted from continuous system bottlenecks.
	
Besides stochastic stragglers, there can be persistent stragglers due to network heterogeneities~\cite{DBLP:conf/mlsys/ChoF0H19, DBLP:conf/mlsys/LuoWKCN20} and contentions~\cite{DBLP:conf/sigcomm/XieDHK12,DBLP:conf/sigcomm/LeeTLPBKS14} in the real GPU cluster or cloud environment. In a crowded platform, the workers of one DML task are often scatter allocated in different racks and even pods. Therefore, some links crossing upper-level switches have to suffers from oversubscriptions and larger latency, while most links are within the same region. Additionally, there are usually many tasks running simultaneously on the platform. Those tasks may share network links or nodes and compete for network bandwidth~\cite{DBLP:conf/sigcomm/XieDHK12,DBLP:conf/sigcomm/LeeTLPBKS14}. Obviously, the network heterogeneity and contention can last for many iterations so that stragglers due to those network bottlenecks are persistent, which relaxed synchronization cannot handle. What is worse, the consistent and accumulated high-level staleness of persistent stragglers brings difficulties for those works to converge properly. 

To this point, we propose Divide-and-Shuffle Synchronization (DS-Sync) to combat those persistent stragglers due to network bottlenecks. Motivated by the observation (details in Section~\ref{sec:sync_scale}) that synchronizing more workers takes more time, DS-Sync divides all workers into independent groups of different sizes to synchronize in parallel. It keeps stragglers in the smaller group, while other fast workers form larger groups to avoid idle waiting. With less latency and transfer cost, small groups with straggler can catch up and may keep the same pace with other large groups consisting of fast workers. 

To maintain the convergence, DS-Sync shuffles the group members in a designed pattern in every iteration. Therefore, any worker can synchronize parameters with unseen workers from other groups in the last iteration. Intuitively, shuffling enables every worker to get the global update information from all workers in certain iterations instead of every iteration. In Section~\ref{sec:convergence}, we formally prove that DS-Sync converges in non-convex and smooth situations like DNNs without convergence speed loss. What is more, we can further extend weight average~\cite{DBLP:conf/uai/IzmailovPGVW18} to ensemble the diverse local models for better generalization performance. We have implemented DS-Sync in the Pytorch framework and verify its improvements by experiments.  In Fig~\ref{fig:ds_sync}, we compare our DS-Sync with BSP and gossip in a toy example to show the advantages in system throughput.

 \begin{figure*}[ht]
  	\centering
  	\includegraphics[scale=0.55]{figures/ds_sync.pdf}
  	\caption{Comparison in 8 workers with the slow link(red dash line): (a) Ring-AllReduce suffers from the bottleneck that affects global synchornization on all workers. (hierarchical Ring-AllReduce~\cite{DBLP:conf/mlsys/ChoF0H19,DBLP:journals/corr/abs-1807-11205} can help but has three serial steps: reduce, reduce and broadcast.)  (b) In Gossip example, every worker(e.g., 1\#) receives from last(e.g., 0\#) and next(e.g., 2\#) neighbors simultaneously and suffers from the in-cast problem. The overlapped part of Dec-Sync will be the new bottleneck if forming irregular neighborhoods. (c) DS-Sync divides workers into independent groups without overlapping and shuffles group members every iteration. It reduces transfer delay and latency for persistent stragglers by forming the smaller group. }
  	\label{fig:ds_sync}
  \end{figure*}

Overall, we propose DS-Sync for DML to reduce training wall-time by alleviate persistent stragglers due to network bottlenecks. In summary,  DS-Sync makes 3-fold contributions as the follows:
\begin{enumerate}
	\item We propose the DS-Sync that divides and shuffles workers into parallel groups to synchronize independently instead of the global synchronization. DS-Sync further schedules workers to form groups of different sizes and keep stragglers in the smaller groups to have less synchronization cost and catch up. 
    \item We formally prove that DS-Sync converges properly on training data in non-convex and smooth situations like DNN. If not much better, the extended ensemble strategy at least help maintain the same generalization performance on test data.
    \item We implement DS-Sync in the pytorch framework and verify the improvements by comprehensive experiments. Empirical study shows DS-Sync can achive speed up as high as 2 times compared with baselines.
 \end{enumerate}
